Modelling cosmological singularity with compactified Milne space

Recent developments in observational cosmology call for understanding the nature of the cosmological singularity (CS). Our work proposes modelling the vicinity of CS by a time dependent orbifold (TDO). Our model makes sense if quantum elementary objects (particle, string, membrane) can go across the singularity of TDO, and our work addresses this issue. We find quantum states of elementary objects, that can propagate in TDO. Our results open door for more detailed examination.

==> ABS.tex <==
% Thesis Abstract ------------------------------------------------------

\prefacesection{Abstract}


Recent developments in observational cosmology call for
understanding the nature of the cosmological singularity (CS). Our
work proposes modelling the vicinity of CS by a time dependent
orbifold (TDO). Our model makes sense if quantum elementary
objects (particle, string, membrane) can go across the singularity
of TDO, and our work addresses this issue. We find quantum states
of elementary objects, that can propagate in TDO. Our results open
door for more detailed examination.
% ----------------------------------------------------------------------

